Voting for the right answer: Adversarial defense for speaker verification

Automatic speaker verification (ASV) is a well developed technology for biometric identification, and has been ubiquitous implemented in security-critic applications, such as banking and access control. However, previous works have shown that ASV is under the radar of adversarial attacks, which are very similar to their original counterparts from human's perception, yet will manipulate the ASV render wrong prediction. Due to the very late emergence of adversarial attacks for ASV, effective countermeasures against them are limited. Given that the security of ASV is of high priority, in this work, we propose the idea of "voting for the right answer" to prevent risky decisions of ASV in blind spot areas, by employing random sampling and voting. Experimental results show that our proposed method improves the robustness against both the limited-knowledge attackers by pulling the adversarial samples out of the blind spots, and the perfect-knowledge attackers by introducing randomness and increasing the attackers' budgets.

==> interspeech 2021/abstract.tex <==
\begin{abstract}
%Automatic speaker verification(ASV) now is a matured technology and has been adopted in a wide range of security-critic applications. However, the unprotected ASV system may suffer from deliberately generated spoofing audio in particular adversarial attack. 
%In this paper, we propose a voting method to improve the robustness of ASV system 
Automatic speaker verification (ASV) is a well developed technology for biometric identification, and has been ubiquitous implemented in security-critic applications, such as banking and access control.
However, previous works have shown that ASV is under the radar of adversarial attacks, which are very similar to their original counterparts from human's perception, yet will manipulate the ASV render wrong prediction.
Due to the very late emergence of adversarial attacks for ASV, effective countermeasures against them are limited.
Given that the security of ASV is of high priority, in this work, we propose the idea of ``voting for the right answer" to prevent risky decisions of ASV in blind spot areas, by employing random sampling and voting.
Experimental results show that our proposed method improves the robustness against both the limited-knowledge attackers by pulling the adversarial samples out of the blind spots, and the sufficient-knowledge attackers by introducing randomness and increasing the attackers' budgets.
% The code is available for reproducing main results.



\end{abstract}

% Yang Zhang
% However, previous researches shows that the unprotected ASV system may suffer from deliberately spoofing audio, in particular adversarial attack, which have 99% similar to their ground truth audio and will manipulate the ASV render wrong prediction.

==> interspeech 2021/background.tex <==
\section{Background}

\subsection{Automatic Speaker verification}
ASV aims to determine whether a piece of given speech belongs to an alleged speaker.
Given an enrollment and test utterance, $x_{e}$ and $x_{t}$, the ASV model will certify whether they are pronounced by the same speaker.
Specifically, the procedure of ASV can be divided into three steps: firstly feature engineering which maps the audio waveform to acoustic features, secondly speaker embedding extraction which extracts the fixed-dimensional speaker embeddings from the variable-length acoustic feature sequences, and finally a back-end model that measures the similarity between speaker embeddings.
%A simple cosine distance can be used for this similarity comparison. In addition, a more complicated scoring back-end can be trained such as Probabilistic Linear Discriminant Analysis(PLDA)\cite{ioffe2006probabilistic} to generate scoring functions.
For brevity, the three steps can be denoted by a scoring function $f$:
\begin{align}
    &s = f(x_{t}, x_{e}), \label{eq:score}
\end{align}
where, $x_{t}$ and $x_{e}$ are the test and enroll utterance, respectively; $s$ measures the similarity between $x_t$ and $x_e$.
The smaller $s$ is, the less likely they belong to the same person, and vice versa.

\subsection{Adversarial attack}
Adversarial samples are generated by slightly modifying the genuine samples with deliberately crafted perturbations.
% , and harnessing adversarial samples to attack machine learning models is called as adversarial attack. 
The deliberately crafted perturbations are usually indistinguishable from human's perception, yet significantly change the output of the model.
Different strategies to generate the adversarial noise result in different attack algorithms, and in this paper, we adopt Basic Iterative Method (BIM) \cite{kurakin2016adversarial}, an efficient iterative adversarial attack method.
In BIM, attackers initialize $x_{t}^{0}=x_{t}$, where $x_{t}$ means the testing utterance in Eq.~\ref{eq:score},then iteratively update it as this equation:
\begin{equation}
\begin{aligned}
    x_{t}^{n+1}=Clip_{\epsilon}^{x_{t}}\left(x_{t}^{n}+\alpha \cdot \lambda \cdot sign\left(\nabla_{x_{t}^{n}}f(x_{t}^{n}, x_{e}) \right)\right), 
    \\ for \, n=0,1, \ldots, N-1,
\end{aligned}
\end{equation}
where $Clip(.)$ is a clipping  operation that ensures $||x_{t}^{n+1} - x_{t}||_{\infty}\leq \epsilon$, $\epsilon \geq 0$ and $\epsilon \in \mathbb{R}$, $\alpha$ is the step size, $\lambda=1$ for the non-target trial and $\lambda=-1$ for the target trial, and $N$ is the number of iterations.
$\epsilon$ determines the attack intensity which is a predefined value by attackers.
In the target trial, the testing and enroll speech are uttered by the same speaker, while in the non-target trial, they are generated by different speakers.
For example, if the attacker want to attack ASV for the non-target trial, they will adopt BIM to make the similarity score between the testing and enrollment speech as high as possible in order to let the ASV model falsely accept the imposter.

\subsection{System evaluation metrics}
The testing trials can be represented as: $\mathbb{T}=\mathbb{T}_{tgt} \cup \mathbb{T}_{ntgt}$, where $\mathbb{T}_{tgt}$ and $\mathbb{T}_{ntgt}$ denote the target trials and non-target trials respectively.
We divide the testing trials into two sets, $\mathbb{T}=\mathbb{D} \cup \mathbb{E}$, where $\mathbb{D}=\mathbb{D}_{tgt} \cup \mathbb{D}_{ntgt}$ is the development set, $\mathbb{E}=\mathbb{E}_{tgt} \cup \mathbb{E}_{ntgt}$ is the evaluation set.
We determine the decision threshold $\tau_{ASV}$ by the development set as below:
\begin{align}
    &DevFAR(\tau) = \frac{\vert \{s_i \geq \tau : i \in \mathbb{D}_{ntgt}\} \vert}{\vert \mathbb{D}_{ntgt} \vert} \label{eq:gen-far} \\
    &DevFRR(\tau) = \frac{\vert \{s_i < \tau : i \in \mathbb{D}_{tgt}\} \vert}{\vert \mathbb{D}_{tgt} \vert} \label{eq:gen-frr} \\
    &\tau_{ASV} = \{ \tau \in \mathbb{R} : DevFAR(\tau) = DevFRR(\tau) \} \label{eq:asv-threshold} 
    % &GenEER = GenFAR(\tau_{ASV}) = GenFRR(\tau_{ASV}) \label{eq:gen-eer}
\end{align}
where $DevFAR(\tau)$ and $DevFRR(\tau)$ mean the development false acceptance rate and false rejection rate respectively under the decision threshold $\tau$, $\mathbb{D}_{tgt}$ and $\mathbb{D}_{ntgt}$ denote the development trial sets containing target and non-target trials, respectively, $s_i$ is the ASV score for the trial $i$ and $\vert \mathbb{A} \vert$ denotes the number of elements in set $\mathbb{A}$. 

Then we evaluate the ASV performance on evaluation set, by FAR and FRR:
\begin{align}
    &FAR = \frac{\vert \{s_i \geq \tau_{ASV} : i \in \mathbb{E}_{ntgt} \} \vert}{\vert \mathbb{E}_{ntgt} \vert} \label{eq:adv-far} \\
    &FRR = \frac{\vert \{ s_i < \tau_{ASV} : i \in \mathbb{E}_{tgt} \} \vert}{\vert \mathbb{E}_{tgt} \vert} \label{eq:adv-frr}
\end{align}
% zyz
% where $\tau_{ASV}$ is the system decision threshold determined by Eq.~\ref{eq:asv-threshold}.
where $\tau_{ASV}$ is the decision threshold determined by Eq.~\ref{eq:asv-threshold}.

==> interspeech 2021/conclusion.tex <==
\section{Conclusion}

% This paper we proposed a voting based method for adversarial defense in deep speaker verification system.
% We adopt data augmentation by add random Gaussian noise during inference, the experimental results show that our method achieve effective defense performance even the attackers know the system defense method.
% Since our approach is every simple but effective for adversarial defense, we are convinced that voting method can be a strong comparable baseline for other novel adversarial defense method.
% Voting strategy also can combine with other defense algorithm to achieve better performance.
% We will open source the code if this paper is accepted.

In this paper, we propose the idea of ``voting for the right answer" to prevent risky decisions of ASV in blind spot areas, by employing random sampling and voting.
Experimental results show our proposed method can both counter limited-knowledge attackers, and sufficient-knowledge attackers with more attack budgets.
We opened source the code 
\footnote[2]{\url{https://github.com/thuhcsi/adsv_voting}} to make our method a comparable baseline.
%\footnote[2]{\href{https://github.com/thuhcsi/adsv_voting}{\texttt{Code}}} to make our method a comparable baseline.
Future work will be dedicated to investigate other sample strategies e.g., sampling within the phone subspace, rather than the blind Gaussian to improve the defense performance of the voting strategy.
We are not familiar with adaptive attacks \cite{tramer2020adaptive} when writing this paper. We will refer to  \cite{yang2020characterizing} and dedicate efforts to invest more powerful adaptive attacks in the future work.

\section{Acknowledge}
This work was done when H. Wu was a visiting student at Shenzhen International Graduate School, Tsinghua University. H. Wu is supported by Frontier Speech Technology Scholarship of National Taiwan University. Y. Zhang is supported by National Natural Science Foundation of China (NSFC) (62076144) and joint research fund of NSFC-RGC (Research Grant Council of Hong Kong) (61531166002, N$\_$CUHK404/15).

% Note that our method didn't take the adaptive attacks into account, and we will invest and improve the performance of our method under adaptive attacks in the future work.

==> interspeech 2021/experiment.tex <==
\section{Experimental setup}
\label{sec:exp_setup}


\subsection{Data}

Voxceleb 1\&2 datasets \cite{nagrani2017voxceleb,chung2018voxceleb2} are used in our experiments.
We train models on the development set of VoxCeleb 1\&2. 
To test our ASV system, we use the trials provide in VoxCeleb1 test set, which contains 37,720 enrollment-testing pairs.
To conduct the experiment more rigorously and without loss of generality, we randomly select 27,720 trails as development set to evaluate the performance of our ASV system on genuine samples and determine the decision threshold in Eq.~\ref{eq:asv-threshold}, and the rest 10,000 trials are left as the evaluation set for generating adversarial samples and evaluating defense performance.

\subsection{ASV system setup}


We build our ASV systems following \cite{chung2020in}, using \textbf{Fast ResNet-34} model structures and angular margin (AM) loss.
Self-Attentive Pooling (\textbf{SAP}) \cite{zhu2018self} and Attentive Statistics Pooling (\textbf{ASP}) \cite{okabe2018attentive} are used to aggregate frame-level features into utterance-level representations.
\textbf{SAP} and \textbf{ASP} denote these two systems in the following description.
In our experiments, we set the hyperparameters of AM loss $scale$ as 30 and $margin$ as 0.1.
% Please see \cite{chung2020in} for more details.
The models are trained for 50 epochs by the Adam optimizer with an initial learning rate of 0.01 decreasing by 10\% every 2 epochs.
During training, we use 2-second fixed length audio segments, extracted randomly from each utterance, and the batch size is 200. 
Spectrograms are extracted with a hamming window of width 25ms and shift 10ms, and 64-dimensional FBanks are used as the models' inputs. 
Our focus is countering the adversarial noise, rather than obtaining state-of-the-art ASV system. Therefore, no data augmentation and voice activity detection are conducted during training, and we use cosine distance for scoring.
Our model achieved 2.52\% equal error rate with ASP and 2.58\% with SAP in development set. 
We determine and fix the models' decision thresholds $\tau_{ASV}$ by Eq.~\ref{eq:asv-threshold}.



\subsection{BIM attack setup}
We generate adversarial samples by BIM. 
In our experiments, we fix the number of iterations $N$ as 5, set the step size $\alpha$ as $\epsilon$ divided by $N$, and use different settings of $\epsilon$: 1,5,10. 
The ASV systems' performance are reported in Table \ref{table:attack_results}. 
After attack, FAR and FRR increase drastically, which shows the effectiveness of BIM.
%The larger $\epsilon$ is, the more intense of the attack.
The larger $\epsilon$ is, the worse of the ASV performance, indicating more intense the attack is.


\begin{table}[h]
\centering
% \caption{BIM attack results in evaluation trial set}
% \vspace{-5pt}
\caption{ASV performance for genuine and adversarial samples}
% \vspace{-10pt}
\begin{tabular}{cccccc}
\hline
\multicolumn{2}{c}{}       & No attack & $\epsilon=1$ & $\epsilon=5$ & $\epsilon=10$ \\ \hline
\multirow{2}{*}{\textbf{ASP}} & FAR & 2.24      & 18.38        & 71.83        & 89.38         \\
                     & FRR & 2.56      & 20.17        & 74.92        & 91.94         \\ \hline
\multirow{2}{*}{\textbf{SAP}} & FAR & 2.35      & 18.43        & 72.11        & 89.55         \\
                     & FRR & 2.23      & 20.21        & 74.33        & 91.7          \\ \hline
\end{tabular}
% \vspace{-10pt}
\label{table:attack_results}
\end{table}

\section{Experimental results}
% In this section, we report our experiments results.
\label{sec:exp_result}

\subsection{Defense for limited-knowledge attackers}


\begin{table*}[t]
\centering
\caption{Defense performance against Limited-knowledge attackers}
% \vspace{-10pt}
\resizebox{\textwidth}{17mm}{
\begin{tabular}{cccccccccccc}
\hline
\multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{\multirow{2}{*}{No defense}} & \multicolumn{1}{l}{\multirow{2}{*}{Gaussian}} & \multicolumn{1}{l}{\multirow{2}{*}{Mean}} & \multicolumn{1}{l}{\multirow{2}{*}{Median}} & \multicolumn{6}{c}{Voting}                                                                  \\
                     &                      & \multicolumn{1}{l}{}                            & \multicolumn{1}{l}{}                          & \multicolumn{1}{l}{}                      & \multicolumn{1}{l}{}                        & $\sigma=1$    & $\sigma=15$ & $\sigma=30$   & $\sigma=60$    & $\sigma=90$ & $\sigma=120$   \\ \hline
\multirow{4}{*}{FAR} & No attack            & 2.24                                            & 1.88                                          & 2.69                                      & 0.98                                        & 2.25          & 2.32        & 2.16          & 2.14           & 1.84        & 1.61           \\
                     & $\epsilon=1$         & 18.38                                           & 11.47                                         & 12.47                                     & 1.85                                        & 16.36         & 27.33       & 2.89          & 2.42           & 2.13        & \textbf{1.83}  \\
                     & $\epsilon=5$         & 71.83                                           & 56.86                                         & 59.66                                     & 6.3                                         & 70.83         & 27.55       & 10.62         & 4.63           & 3.05        & \textbf{2.54}  \\
                     & $\epsilon=10$        & 89.38                                           & 80.7                                          & 82.89                                     & 12.35                                       & 89.13         & 69.2        & 29.66         & 9.43           & 5.32        & \textbf{3.6}   \\ \hline
\multirow{4}{*}{FRR} & No attack            & 2.56                                            & 3.04                                          & 2.05                                      & 19.55                                       & 2.27 & 2.82        & 3.32          & 4.95           & 6.06        & 8.12           \\
                     & $\epsilon=1$         & 20.17                                           & 17.38                                         & 14.77                                     & 24.24                                       & 16.59         & 4.9         & \textbf{4.53} & 5.33           & 6.98        & 8.76           \\
                     & $\epsilon=5$         & 74.92                                           & 62.22                                         & 65.47                                     & 40.8                                        & 72.79         & 33.56       & 16.78         & \textbf{10.74} & 10.81       & 12.18          \\
                     & $\epsilon=10$        & 91.94                                           & 87.58                                         & 87.13                                     & 55.42                                       & 91.1          & 73.74       & 42.52         & 21.77          & 17.05       & \textbf{16.67} \\ \hline
\end{tabular}
}
\label{tab:defense_results}
% \vspace{-15pt}
\end{table*}

%This scenario is more practical as the attackers usually can't access to the defense method. 
%This scenario is more practical as the attackers usually can't have access to the defense method. 
In this scenario, the attackers can access the ASV model, but do not know the defense method.
There is few baseline for reference and in order to make a clear comparison, we follow our previous work \cite{wu2021adversarialasv} which applies hand-crafted filters including Gaussian filter, mean filter and median filter for adversarial defense, and set them as our baseline. 
We use different settings of the voting variance $\sigma$, randomly sample 50 neighbors around the testing audio, and let the neighbors vote for whether the utterance should be accepted or not.
The performance with \textbf{SAP} exhibits a similar trend as with \textbf{ASP}, and due to limited space, we only report the results of \textbf{ASP}.
In Table~\ref{tab:defense_results}, we evaluate the FAR and FRR of different defense methods, and note that the FAR and FRR for voting is calculated as Eq.~\ref{eq:vote-far} and Eq.~\ref{eq:vote-frr}.
We evaluate both the negative effects of the defense methods for genuine samples (rows labeled by No attack), 
%and the defense performance for adversarial samples in different settings of $\epsilon$.
and the positive effects on adversarial samples in different settings of $\epsilon$.
The observations and analysis are concluded as follows:
(1) Gaussian, mean and the voting method with different $\sigma$ slightly affect the FAR and FRR of genuine samples, while median filter enlarges the FRR from 2.56\% to 19.55\%, indicating that median filter highly distorts the speech signal.
(2) The three filter-based models help alleviate the adversarial attacks, but the defense performance of them is greatly outperformed by the voting-based defense.
%What's more, as $\epsilon$ become large, the three filters can slightly counter the adversarial noise, while the voting based method still decrease FAR and FRR to a great deal.
What's more, as $\epsilon$ become large, the performances of the three filter-based methods are significantly degraded, while the voting based method still decrease FAR and FRR to a great deal.
(3) Note that when $\sigma$ is small, the voting strategy can't alleviate the adversarial noise, as the neighbors are still with large probability in the blind spot as claimed in Section~\ref{sec:vote_works}.
And when $\sigma$ increases, the FAR and FRR drop drastically, as a large proportion of neighbors are outside the blind spot and they will vote for the right answer.
%\footnote{We put some samples in \href{https://zyzisyz.github.io/voting\_audio\_samples}}

\begin{figure}[h]
  \centering
%   \vspace{-5pt}
  \centerline{\includegraphics[width=6cm]{figures/num_votes_1.png}}
%   \vspace{-8pt}
  \caption{Defense performance in different number of votes}
  \label{fig:num_votes}
%   \vspace{-8pt}
\end{figure}

Fig.~\ref{fig:num_votes} shows FAR and FRR on genuine samples (a and c) and adversarial samples (b and d) with different number of votes, $K$, given $\epsilon = 5$.
We observe that:
(1) When the number of votes increases, the FAR and FRR for adversarial samples drops drastically.
And when $K$ is around 10, the FAR and FRR for adversarial samples become saturated, which means we can use about 10 votes to achieve effective defense performance.
(2) Fig.~\ref{fig:num_votes}.c shows as $K$ increases, the FRR on genuine samples increases, which means the voting strategy results in negative effect on genuine samples. However, this is just a mild negative effect outweighed by the performance improvement on adversarial samples.
We can choose a reasonable number $K$ to balance the trade-off between the negative effect on genuine samples and positive effect on adversarial samples, 
which take the system security and user experience into consideration according to the system requirements.



\subsection{Defense for sufficient-knowledge attackers}

In this subsection, we give a case study to evaluate the robustness of our method under a more extreme scenario, where attackers have sufficient knowledge in particular the defense method.
%We imitate the attackers and the BIM objective becomes increasing and decreasing $s_{vote}$ in Eq.~\ref{eq:vote-score} for non-target and target trials, respectively.
Sufficient knowledge BIM aims to attack not only
the original sample, but also its $K$ neighbors which are randomly sampled for voting.
Therefore, the new BIM against voting defense requires around $K+1$ times computing resource compared to the original BIM counterpart, however it's hard to accomplish by our computing resource when $K$ is too large \footnote[1]{This indicates when attackers have sufficient knowledge, the cost of attacking the system would increase.}.
So we just set the number of votes as 5 to illustrate a case study.
We fix $\epsilon$ as 5, attack iteration $N$ as 5, and $\sigma$ as 60.
For filter-based defense methods, the sufficient-knowledge attackers view the ASV system equipped with hand-crafted filters as an entire system, and directly get the gradient of such system and attack it.
Due to limited space, we only show the results of Gaussian filter, and the other filters are with the same trends.
Table~\ref{tab:perfect} reports the results.
%Note that the performance of limited knowledge attackers is different from Table~\ref{tab:defense_results} as votes are different.
Note that the performance of limited knowledge attackers in Table~\ref{tab:perfect} is worse than Table~\ref{tab:defense_results} because the numbers of votes are different.
We observe that:
(1) The voting based method achieves better defense performance than Gaussian filter.
(2) Though the attackers know the voting defense and use more computing resource, they still can't do attack effectively, as the FAR and FRR only increase slightly.


\begin{table}[ht]
% \vspace{-5pt}
\setlength\tabcolsep{4pt}
\centering
\caption{Defense results for sufficient-knowledge attackers }
% \vspace{-10pt}
\begin{tabular}{cccccc}
\hline
\multirow{2}{*}{} & \multirow{2}{*}{No defense} & \multicolumn{2}{c}{Gaussian} & \multicolumn{2}{c}{Voting} \\
                  &                             & limited       & sufficient      & limited      & sufficient     \\ \hline
FAR(\%)               & 71.83                       & 56.86         & 60.13        & 10.66        & 13.29       \\ \hline
FRR(\%)               & 74.92                       & 62.22         & 64.53        & 24.68        & 27.75        \\ \hline
\end{tabular}
% \vspace{-5pt}
\label{tab:perfect}
\end{table}

Furthermore, Fig.~\ref{fig:iter} shows the attack results when the attack iteration $N$ increases, which means the attackers get more attack budgets by enlarging $N$.
However, as $N$ becomes larger than 10, the values of FAR and FRR become saturated.
This is another evidence to show the effectiveness of the voting based defense method, as it introduces randomness and obfuscates the gradient based attack algorithm.


\begin{figure}[ht]
  \centering
%   \vspace{-5pt}
  \centerline{\includegraphics[width=6cm]{figures/iter_1.png}}
%   \vspace{-5pt}
  \caption{Attack performance with different $N$}
  \label{fig:iter}
%   \vspace{-5pt}
\end{figure}






==> interspeech 2021/introduction.tex <==



\section{Introduction}
\label{sec:intro}
% ASV aims at verifying whether a certain speaker pronounces a piece of given utterance.
Automatic speaker verification (ASV), is to determine whether a claimed identity is speaking during a speech segment \cite{zheng2017robustness}.
Thanks to previous efforts \cite{kenny2007joint,dehak2010front,li2017deep,snyder2018x}, ASV is now a well-developed technology for biometric identification and widely adopted in various security-critic applications.
But, ASV models with high performance are vulnerable to spoofing audios \cite{todisco2019asvspoof} generated by audio replay, text-to-speech and voice conversion, back-door attacks \cite{zhai2021backdoor}, and related emerged adversarial attacks \cite{kreuk2018fooling,das2020attacker}.
% The ASVspoof challenge series \cite{wu2015asvspoof,kinnunen2017asvspoof,todisco2019asvspoof} arouses the attention from the industry and academia and high performance countermeasures against spoofing audios have been proposed.
% The ASVspoof challenge series \cite{wu2015asvspoof,kinnunen2017asvspoof,todisco2019asvspoof} address the spoofing audios and effective countermeasures against them have been proposed.
In this paper, we mainly focus on tackling the adversarial attacks.

Adversarial samples were first raised by \cite{szegedy2013intriguing} and they regarded them as blind spots of models.
Harnessing adversarial samples to attack well-trained models is \emph{adversarial attack}.
Adversarial samples are generated by slightly modifying the genuine samples with deliberately crafted perturbations, and \cite{szegedy2013intriguing} shows that such elaborated samples can manipulate image classification models with high performance predict wrong answers.
% This phenomenon is particularly surprising as the modiﬁcation is often imperceptible and we, humans, can't distinguish the genuine sample and its modified adversarial counterpart.
% This phenomenon is particularly surprising as humans, can't distinguish the genuine sample and its modified adversarial counterpart.
Also, audio processing models are vulnerable to adversarial attacks.
Carlini and Wagner \cite{carlini2018audio} shows that adversarial attacks can hallucinate state-of-the-art automatic speech recognition (ASR) model.
% Given a piece of audio, either speech, silence, or music, \cite{carlini2018audio} can generate another over 99\% similar adversarial counterpart, which can manipulate the ASR transcript any text predefined by the authors.
Given a piece of audio, either speech, silence, or music, \cite{carlini2018audio} can generate another perceptually indistinguishable adversarial sample, which can deceive the ASR output text predefined by the attackers.
% \cite{yuan2018commandersong,schonherr2018adversarial,yakura2018robust,taori2019targeted,qin2019imperceptible} also illustrate the vulnerability of ASR models from different perspectives.
The vulnerability of ASR to adversarial attacks has been also studied by \cite{yuan2018commandersong,schonherr2018adversarial,yakura2018robust,qin2019imperceptible}.
Other audio processing tasks, such as anti-spoofing for ASV \cite{liu2019adversarial,wu2020defense_2,wu2020defense}, voice conversion \cite{huang2021defending} and sound event classification \cite{subramanian2019robustness}, are also subject to adversarial attacks.

The performance of ASV will drop catastrophically under adversarial attacks \cite{kreuk2018fooling,li2020adversarial,xie2020real,marras2019adversarial,li2020practical,chen2019real,wang2020inaudible,villalba2020x,das2020attacker}.
\cite{kreuk2018fooling} firstly shows ASV is subject to adversarial attacks.
% \cite{chen2019real} attack ASV with few speakers.
\cite{chen2019real} attacks ASV trained by only a few speakers.
\cite{villalba2020x} and \cite{li2020adversarial} respectively show the vulnerability to adversarial attacks of i-vector and x-vector models.
Recently, researchers also investigated more risky adversarial attacks which are inaudible \cite{wang2020inaudible} and universal \cite{marras2019adversarial,xie2020real}, and can spread over the air \cite{li2020practical,xie2020real}.
% \cite{marras2019adversarial} investigate the universality of adversarial attack by crafting master voices, which can imitate a large proportion of enrolled users.
% Wang et al. \cite{wang2020inaudible} craft more inaudible adversarial audios by harnessing the psychoacoustic principle \cite{lin2015principles}.
% Li et al. \cite{li2020practical} first demonstrate the possibility of over-the-air adversarial attacks against x-vector system in the physical world.
% The first audio-independent and over-the-air adversarial noise is proposed to fool the x-vector system \cite{xie2020real}. 
% With ubiquitous usage of ASV in safety-critical environment, equipping ASV with the robustness against adversarial attacks is indispensable.
Only limited works \cite{wang2019adversarial,li2020investigating,zhang2020adversarial,wu2021adversarialasv} are conducted to protect ASV from adversarial attacks.
So it is still an open question to effectively tackle this issue.
% \cite{zhang2020adversarial} trains an DNN based filter by the training dataset consists of both genuine and adversarial samples, to alleviate the adversarial noise.
\cite{zhang2020adversarial} trains a deep neural network based filter to eliminate adversarial noise.
% by the training dataset consisting of genuine and adversarial samples.
A binary classification model \cite{li2020investigating} is trained to spot the adversarial samples.
\cite{wang2019adversarial} adopts adversarial training  to improve the robustness of ASV.
% which injects the adversarial samples into training data to improve the robustness of ASV.
Self-supervised learning based filters are used to alleviate the adversarial noise for ASV \cite{wu2021adversarialasv,wu2021adversarial-2}.

In this paper, we propose to improve the adversarial robustness by sampling the neighbors of a given utterance and letting the neighbors vote for whether the utterance should be accepted or not by the ASV model.
The adversarial samples are blind spots of ASV and we believe the radius of such blind spots is small, as shown in Table~\ref{tab:defense_results}.
So if the spread of the sample space is large, then there is a large probability that most of the neighbours are outside of the blind spot. 
In this case, the voting will result in the right decision.
Contrary to \cite{wang2019adversarial,li2020investigating,zhang2020adversarial} which require the system designers to model the in-the-wild attackers and know exactly the adversarial attack methods adopted during attack in advance, our method is attack-agnostic.
In contrast to \cite{wu2021adversarialasv,wu2021adversarial-2} which counter adversarial noise in the frequency domain, our method is in the time domain.
Our method harnesses the idea of ``voting for the right answer" to let the ASV make the decision based on an utterance's neighbors rather than the utterance itself, thus equips the ASV model with the capacity of countering adversarial attacks.
The experimental results show the effectiveness of our defense method.

% Our contributions are as below.
% We propose an attack-agnostic method, which harnesses the idea of ``voting for the right answer" to let the ASV make the decision based on an utterance's neighbors rather than the utterance itself, thus equips the ASV model with the capacity of countering adversarial attacks.
% The experimental results show the effectiveness of our defense method.
% The experimental results show that our proposed method improves the robustness against both the limited-knowledge attacks by pulling the adversarial samples out of the blind spots, and the perfect-knowledge attackers by introducing randomness and causing the attacking gradient unstable and obfuscated.

% Automatic speaker verification (ASV) is the task to verify whether a piece of speech sample belongs to a certain speaker, which has found a broad range of applications with various of methods.
% Conventional ASV methods are based on statistical models,
% in particular the Gaussian mixture model-universal background
% model (GMM-UBM)\cite{reynolds2000speaker} and the joint factor analysis (JFA)\cite{kenny2007joint} and the i-vector model\cite{dehak2010front}.
% Later, utilizing the power of deep neural network(DNN) to learn from a large amount of data, x-vector model\cite{snyder2018x} proposed by Snyder et al. achieved good performance in various text-independent speaker recognition tasks. 
% The DNN based models have been significantly improved recently,
% in particular by employing better architectures \cite{chung2018voxceleb2,desplanques2020ecapa,ravanelli2018speaker}, pooling approaches \cite{zhu2018self,lai2019attentive,cai2018novel}, and training objectives \cite{zhou2019deep,li2019boundary,gao2019improving,liu2019large}.
% Speaker verification is now a matured technology widely applied to biometric identification.

% Despite of the great performance on existing benchmark datasets, ASV sytems are highly suffer from to spoofing audio which deliberately generated by text-to-speech, voice conversion, and audio replay~\cite{wu2015spoofing,wu2016anti},
% as some malicious attackers mimic a specific target user to deceive the ASV systems.
% Therefore, when ASV systems deploy to real applications,
% strategies to handle the spoofing audio are in need.

% Adversarial attack attempts to fool models by supplying deceptive input,
% which was first raised in computer vision filed by\cite{szegedy2013intriguing}.
% Attackers deliberately generated a tiny perturbation, which is indistinguishable from human’s perception, and combine it with the original sample to generate the new sample, which will manipulate the model give wrong prediction. 
% Recently, the security vulnerability of ASV system to adversarial samples has been widely recognized. 

% Our contributions are as follow:


==> interspeech 2021/ref.tex <==
\section{Introduction}
\label{sec:intro}


Automatic speaker verification (ASV) is the task to verify whether a piece of speech sample belongs to a certain speaker, which has found a broad range of applications with various of methods.
Conventional ASV methods are based on statistical models,
in particular the Gaussian mixture model-universal background
model (GMM-UBM)\cite{} and the joint factor analysis (JFA)\cite{} and the i-vector model\cite{}.
Later, utilizing the power of deep neural network(DNN) to learn from a large amount of data, x-vector model\cite{snyder2018x} proposed by Snyder et al. achieved good performance in various text-independent speaker recognition tasks. 
The DNN based models have been significantly improved recently,
in particular by employing better architectures \cite{}, pooling approaches \cite{}, training objectives \cite{}, and training schemes \cite{}.
Speaker verification is now a matured technology widely applied to biometric identification.

Recently, the security vulnerability of DNN models to adversarial samples has been widely recognized. Despite of the great performance on existing benchmark datasets, ASV sytems are highly suffer from to spoofing audio which deliberately generated by text-to-speech, voice conversion, and audio replay~\cite{wu2015spoofing,wu2016anti},
as some malicious attackers mimic a specific target user to deceive the ASV systems.
Therefore, when ASV systems deploy to real applications,
strategies to handle the spoofing audio are in need.

The ASVspoof challenge series \cite{wu2015asvspoof,kinnunen2017asvspoof,todisco2019asvspoof} is a community-driven challenge to arouse attention in addressing spoofing audio attacks and their countermeasures. 
Spoofing countermeasure models, also known as anti-spoofing models, are shields for ASV to detect and filter spoofing audio.
% They only allow the bonafide audio to pass through and finish the ASV task.
Recently several high performance anti-spoofing models have been proposed \cite{evans2013spoofing,Todisco_2016,delgado2018asvspoof,wu2012study,chen2015robust,chen2017resnet,qian2016deep,lai2019attentive,lavrentyeva2019stc,lai2019assert}.

Since Szegedy et al. \cite{szegedy2013intriguing} first proposed the concept of adversarial attacks, and illustrate how deep neural networks with impressive performance for computer vision tasks are vulnerable to adversarial attacks, a large variety of research in this domain have been done.
Adversarial example, which is generated by adding imperceptible perturbation to the input sample, can result in the incorrect prediction of the models.
The added perturbation is carefully crafted such that humans can not distinguish the adversarial example from the input sample visually or acoustically.
Attacking the models with adversarial examples is called adversarial attack.
Previous works show that deep neural networks for speech processing tasks are subject to adversarial attacks. 
\cite{carlini2018audio} investigates the vulnerability of automatic speech recognition (ASR) models to adversarial attacks.
Given any audio waveform, whether speech or music, they can generate an adversarial example, which is over 99\% similar to the original audio but makes the ASR model wrongly predict any transcribes they defined before. 
It has also been shown that ASV systems can be fooled by adversarial examples \cite{kreuk2018fooling,das2020attacker,fli2020adversarial}.
Moreover, in \cite{wu2020defense,liu2019adversarial}, the authors illustrate the anti-spoofing models for ASV systems are also vulnerable to adversarial attacks.
In this paper, we focus on the defense for adversarial attacks of the anti-spoofing models. 

Proactive defense and passive defense are two main categories of defense for the adversarial attacks. 
The former defense aims to train new models to counter the adversarial attacks.
The most famous proactive defense method is adversarial training \cite{goodfellow2014explaining}, which injects the adversarial examples generated by different attack algorithms into the training data.
It is reasonable that the models are robust to specific attack algorithms if the models have already seen the adversarial examples during training.
However, adversarial training is time-consuming and resource-consuming.
What’s more, when defenders do adversarial training, they have no idea which attack algorithm the attackers will take. 
The mismatch between attack algorithms during training and inference will make the models susceptible to adversarial attacks they haven’t seen during training. 

Passive defense methods embrace the advantage of defending adversarial examples generated by all kinds of attacking methods without modifying the model. 
The spatial smoothing, also called as filter, is a passive defense method that counters adversarial attacks \cite{xu2017feature}. 
Gaussian filter, median filter and mean filter are used to defend anti-spoofing models in \cite{wu2020defense}. 
The above three filters are shallow filters to counter the deliberately generated adversarial perturbations. 

In this paper, we propose a simple but very effective passive adversarial defense method by voting strategy.
% In the experiment, we compared the performance of these two filters.
% Wu: talk about more about leveraging unlabeled data
% Liu: ok
% In this work, we use self-supervised models to leverage large amount of unlabeled speech to defense black-box attacks on anti-spoofing models.
%It is well known that task specific labeled data may not always be available, as labels are hard to acquire, costly and requires human annotation.
%However, large amount of unlabeled data like raw speech can be easily accessed and gathered, this allows self-supervised learning to gain benefit through pre-training on large scale unlabeled data.
%Self-supervised learning allows the model to learn high-level and contextualized representations from a large amount of unlabeled data, without the use of any label~\cite{bert}.
%In self-supervised learning, a pre-training task (or auxiliary task) that uses only unlabeled data is formulated, and the model is required to solve such a task.
%While solving the pre-training task, the model is also learning a function that maps input to high-level representations, which can potentially transfer information learned from unlabeled data to downstream tasks.
%Through pre-training models on speech, self-supervised learning based models are able to leverage the knowledge of unlabeled speech, then the performance of downstream speech and language processing (SLP) tasks can be improved dramatically~\cite{mockingjay, cpc, apc}, including phone classification, speaker recognition, and speech recognition.
%In recent literature~\cite{mockingjay, cpc, apc, speech_encoder}, downstream SLP tasks, including phone classification, speaker recognition, and speech recognition, are improved by utilizing self-supervised learned models. 
%However, the robustness of such high-level audio representations learned by self-supervised learning based models against adversarial attacks for anti-spoofing of ASV have not been studied yet.
% In this paper, we show that self-supervised learning models can serve as a deep filter which extracts the pivotal information from the contaminated input spectrograms to counter adversarial attacks. 
%However, the robustness of the high-level representations learned by self-supervised learning based models against adversarial attacks has not been studied yet.


%Adversarial attacks, that are imperceptible to original data but result in incorrect prediction from the anti-spoofing models, are dangerous for anti-spoofing models and for the sake of security, we should detect them at any cost.
%Also, the robustness of the high-level representations learned by self-supervised learning based models against adversarial attacks has not been studied yet.
%In this work, we find that self-supervised learning models can serve as a deep filter which extracts the pivotal information from the contaminated input spectrograms to counter the adversarial attacks.
% and protect anti-spoofing models in the black-box attack scenario.
%To the best of our knowledge, we are among the first ones to adopt the high-level representations extracted by the self-supervised model for the defense of anti-spoofing models in the black-box scenario and the experimental results show the effectiveness of our proposed method.
%We also propose the layerwise noise-to-signal ratio (LNSR), to quantize and measure the effect of deep models in countering adversarial noise.
%We find that the adversarial noise is attenuated layer by layer in the self-supervised learning model.

The paper is organized as follows. In Section 2, we firstly revisit the success of data augmentation method, and then introduce the background of adversarial attack and methods adopted in this paper, after that, we presents the proposed voting method. 
Section 4 reports the experimental setups, results, and analysis. Section 5 shows the conclusion.



==> interspeech 2021/voting.tex <==
\section{Voting for the right answer}


\begin{figure}[ht]
  \centering
  \centerline{\includegraphics[width=7cm]{figures/method.png}}
%   \vspace{-10pt}
  \caption{Proposed framework.}
%   \vspace{-10pt}
  \label{fig:method}
\end{figure}

\subsection{Proposed method}

In this subsection, we only introduce the procedure of our proposed method, and detailed explanation and intuition of why it works will be illustrated in next subsection.
For the sake of simplicity, we omit the enroll utterance $x_{e}$, and denote the testing utterance $x_{t}$ as $x^{0}$.
As shown in Fig.~\ref{fig:method}, a Gaussian ball with $x^{0}$ as the center, and variance ,$\sigma$, as the radius, is constructed.
Then we sample $K$ neighbors around $x^{0}$, and denote $\mathbb{X} = \{x^{0},x^{1}, x^{2}..., x^{K}\}$, where $\mathbb{X}$ means the set consisting of  $x^{0}$ and its $K$ neighbors.
Based on $\mathbb{X}$, $\{s^{0}, s^{1}, s^{2}..., s^{K}\}$, are derived as illustrated in Fig.~\ref{fig:method}.
Then, the derived score for voting, $s^{vote}$ is calculated as below:
\begin{align}
    &s^{vote} = \frac{1}{K+1} \sum_{k=0}^{K} s^{k} \label{eq:vote-score}
\end{align}
Based on  $s^{vote}$, the utterance will be accepted if $s^{vote} > \tau_{ASV}$, and vice versa.
Then the modified FAR and FRR for voting, $FAR_{vote}$ and $FRR_{vote}$, are derived:
\begin{align}
    &FAR_{vote} = \frac{\vert \{s^{vote}_{i} \geq \tau_{ASV} : i \in \mathbb{E}_{ntgt} \} \vert}{\vert \mathbb{E}_{ntgt} \vert} \label{eq:vote-far} \\
    &FRR_{vote} = \frac{\vert \{ s^{vote}_{i} < \tau_{ASV} : i \in \mathbb{E}_{tgt} \} \vert}{\vert \mathbb{E}_{tgt} \vert} \label{eq:vote-frr}
\end{align}
where $s^{vote}_{i}$ is the derived score for voting of the $i_{th}$ utterance.


\subsection{Why ``voting for the right answer" works}
\label{sec:vote_works}
It is hard to guarantee the well-trained ASV model is perfect.
So we can regard the ASV we derived is a slightly skewed mapping function from the data space to the label space, which makes some areas of the input space cannot be well covered by the ASV model.
The uncovered input space can be regarded as blind spots of ASV.
The malicious attackers deliberately try every attempt to find the blind spots and hallucinate the ASV model, and we think that adversarial samples are also blind spots of the ASV model.
Data augmentation is an intuitive way to enrich the model's distribution manifolds to cover the blind spots.
However, exhausting all the data augmentation strategies and making the model fill in all the manifolds of data distribution during training is extremely resource-consuming, not to mention that we can't model all the data augmentation strategies.
So we provide another alternative way to handle the blind spots: voting for the right answer.
In case that the testing sample falls into the blind spot, we propose to randomly sample $K$ samples within a Gaussian ball.
And then we let the neighbors of the testing sample vote for the right answer.
These areas of the blind spots are small in volume as shown in Table~\ref{tab:defense_results}, and when random sampling is conducted, the samples tend to jump out of the blind spots if the sampling variance, $\sigma$, is sufficiently large.
The sampled neighbours are with more probabilities to be in a health area rather than in a blind spot area.
Then after voting, the improved probability of being in a health area leads to improved probability of getting a 'normal' decision.

% In order to equip the ASV model with the capacity of simulating the data distribution, a large scale of training data is implemented to train such a model.
% It is known to all that the more diversify of the data augmentation strategies, the larger dataset and the more powerful model we will derive.
% However, exhausting all the data augmentation strategies and making the model fill in all the manifolds of data distribution during training is extremely resource-consuming, not to mention that we can't model all the data augmentation strategies.
% So we harness the idea of ``voting for the right answer" to conduct data augmentation during inference time and equip the ASV model, which is trained by dataset without data augmentation, with the capacity of modeling the nearly entire distribution.

% As we can't exhaust all the data augmentation strategies, the derived ASV model is unable to fill in all the manifolds of the data distribution, resulting in blind spots of the well-trained ASV model.
% The in-the-wild attackers deliberately make every attempt to find the blind spots and attack the ASV model, and we argue that adversarial samples are also blind spots of the ASV model, which can be adopted to hallucinate the ASV model.
% In case that the testing sample falls into the blind spot, we propose to sample $K$ samples within a Gaussian ball.
% And then we let the neighbors of the testing sample vote for the right answer.
% The spread or the dispersion between the center of the blind spot and its boundary, is usually small as shown in Table~\ref{tab:perfect}, so if the voting sigma, $\sigma$, is highly larger than the spread, it is likely a large proportion of the $K$ samples are outside the blind spot.
% Adopting the samples outside the blind spot for voting is more likely to derive the right answer.
% The qualified voting sigma $\sigma$ and the sample number $K$, should fulfill the requirement of mitigating the adversarial attack effectively without sacrificing the accuracy of genuine samples too much, and we show the procedure of searching for them in Section~\ref{sec:exp_result}.

\subsection{Threat model and our countermeasures}
% Previous works crudely classify the attacking scenarios into white-box or black-box, which is sometimes vague and unclear.
We divide the threat models according to the knowledge obtained by the attackers and followed by our countermeasures.

\textbf{Limited-knowledge attackers}: Limited knowledge attackers have the access to the internals of the target ASV model, including parameters and gradients, but are unaware of the defense method. The attackers elaborate the adversarial samples which are blind spots of ASV. In this scenario, our defense method can choose a suitable $\sigma$ and sample a large proportion of neighbours outside the blind spots, so that we have a large probability to get the right answer by voting.

\textbf{Sufficient-knowledge attackers}: Compared with limited-knowledge attackers, sufficient knowledge attackers even know the defense method.
They do gradient descent to modify the original sample and craft an adversarial counterpart to change the $s_{vote}$ in Eq.~\ref{eq:vote-score} to fool the ASV.
However, we conduct voting during inference and we don't know exactly the neighbors sampled for voting in advance, neither do the attackers. And it is impractical the attackers can exhaust all the possible neighbors for attack, so the exactly gradient for $s_{vote}$ during inference is hard to obtain. The randomness introduced by the voting procedure will hinder and obfuscate the gradient of $s_{vote}$ and make the gradient-based attacks ineffective. Our method attains more potential because we can even determine $\sigma$ and $K$ randomly.


==> ref.tex <==
\section{Introduction}
\label{sec:intro}


Automatic speaker verification (ASV) is the task to verify whether a piece of speech sample belongs to a certain speaker, which has found a broad range of applications with various of methods.
Conventional ASV methods are based on statistical models,
in particular the Gaussian mixture model-universal background
model (GMM-UBM)\cite{} and the joint factor analysis (JFA)\cite{} and the i-vector model\cite{}.
Later, utilizing the power of deep neural network(DNN) to learn from a large amount of data, x-vector model\cite{snyder2018x} proposed by Snyder et al. achieved good performance in various text-independent speaker recognition tasks. 
The DNN based models have been significantly improved recently,
in particular by employing better architectures \cite{}, pooling approaches \cite{}, training objectives \cite{}, and training schemes \cite{}.
Speaker verification is now a matured technology widely applied to biometric identification.

Recently, the security vulnerability of DNN models to adversarial samples has been widely recognized. Despite of the great performance on existing benchmark datasets, ASV sytems are highly suffer from to spoofing audio which deliberately generated by text-to-speech, voice conversion, and audio replay~\cite{wu2015spoofing,wu2016anti},
as some malicious attackers mimic a specific target user to deceive the ASV systems.
Therefore, when ASV systems deploy to real applications,
strategies to handle the spoofing audio are in need.

The ASVspoof challenge series \cite{wu2015asvspoof,kinnunen2017asvspoof,todisco2019asvspoof} is a community-driven challenge to arouse attention in addressing spoofing audio attacks and their countermeasures. 
Spoofing countermeasure models, also known as anti-spoofing models, are shields for ASV to detect and filter spoofing audio.
% They only allow the bonafide audio to pass through and finish the ASV task.
Recently several high performance anti-spoofing models have been proposed \cite{evans2013spoofing,Todisco_2016,delgado2018asvspoof,wu2012study,chen2015robust,chen2017resnet,qian2016deep,lai2019attentive,lavrentyeva2019stc,lai2019assert}.

Since Szegedy et al. \cite{szegedy2013intriguing} first proposed the concept of adversarial attacks, and illustrate how deep neural networks with impressive performance for computer vision tasks are vulnerable to adversarial attacks, a large variety of research in this domain have been done.
Adversarial example, which is generated by adding imperceptible perturbation to the input sample, can result in the incorrect prediction of the models.
The added perturbation is carefully crafted such that humans can not distinguish the adversarial example from the input sample visually or acoustically.
Attacking the models with adversarial examples is called adversarial attack.
Previous works show that deep neural networks for speech processing tasks are subject to adversarial attacks. 
\cite{carlini2018audio} investigates the vulnerability of automatic speech recognition (ASR) models to adversarial attacks.
Given any audio waveform, whether speech or music, they can generate an adversarial example, which is over 99\% similar to the original audio but makes the ASR model wrongly predict any transcribes they defined before. 
It has also been shown that ASV systems can be fooled by adversarial examples \cite{kreuk2018fooling,das2020attacker,fli2020adversarial}.
Moreover, in \cite{wu2020defense,liu2019adversarial}, the authors illustrate the anti-spoofing models for ASV systems are also vulnerable to adversarial attacks.
In this paper, we focus on the defense for adversarial attacks of the anti-spoofing models. 

Proactive defense and passive defense are two main categories of defense for the adversarial attacks. 
The former defense aims to train new models to counter the adversarial attacks.
The most famous proactive defense method is adversarial training \cite{goodfellow2014explaining}, which injects the adversarial examples generated by different attack algorithms into the training data.
It is reasonable that the models are robust to specific attack algorithms if the models have already seen the adversarial examples during training.
However, adversarial training is time-consuming and resource-consuming.
What’s more, when defenders do adversarial training, they have no idea which attack algorithm the attackers will take. 
The mismatch between attack algorithms during training and inference will make the models susceptible to adversarial attacks they haven’t seen during training. 

Passive defense methods embrace the advantage of defending adversarial examples generated by all kinds of attacking methods without modifying the model. 
The spatial smoothing, also called as filter, is a passive defense method that counters adversarial attacks \cite{xu2017feature}. 
Gaussian filter, median filter and mean filter are used to defend anti-spoofing models in \cite{wu2020defense}. 
The above three filters are shallow filters to counter the deliberately generated adversarial perturbations. 

In this paper, we propose a simple but very effective passive adversarial defense method by voting strategy.
% In the experiment, we compared the performance of these two filters.
% Wu: talk about more about leveraging unlabeled data
% Liu: ok
% In this work, we use self-supervised models to leverage large amount of unlabeled speech to defense black-box attacks on anti-spoofing models.
%It is well known that task specific labeled data may not always be available, as labels are hard to acquire, costly and requires human annotation.
%However, large amount of unlabeled data like raw speech can be easily accessed and gathered, this allows self-supervised learning to gain benefit through pre-training on large scale unlabeled data.
%Self-supervised learning allows the model to learn high-level and contextualized representations from a large amount of unlabeled data, without the use of any label~\cite{bert}.
%In self-supervised learning, a pre-training task (or auxiliary task) that uses only unlabeled data is formulated, and the model is required to solve such a task.
%While solving the pre-training task, the model is also learning a function that maps input to high-level representations, which can potentially transfer information learned from unlabeled data to downstream tasks.
%Through pre-training models on speech, self-supervised learning based models are able to leverage the knowledge of unlabeled speech, then the performance of downstream speech and language processing (SLP) tasks can be improved dramatically~\cite{mockingjay, cpc, apc}, including phone classification, speaker recognition, and speech recognition.
%In recent literature~\cite{mockingjay, cpc, apc, speech_encoder}, downstream SLP tasks, including phone classification, speaker recognition, and speech recognition, are improved by utilizing self-supervised learned models. 
%However, the robustness of such high-level audio representations learned by self-supervised learning based models against adversarial attacks for anti-spoofing of ASV have not been studied yet.
% In this paper, we show that self-supervised learning models can serve as a deep filter which extracts the pivotal information from the contaminated input spectrograms to counter adversarial attacks. 
%However, the robustness of the high-level representations learned by self-supervised learning based models against adversarial attacks has not been studied yet.


%Adversarial attacks, that are imperceptible to original data but result in incorrect prediction from the anti-spoofing models, are dangerous for anti-spoofing models and for the sake of security, we should detect them at any cost.
%Also, the robustness of the high-level representations learned by self-supervised learning based models against adversarial attacks has not been studied yet.
%In this work, we find that self-supervised learning models can serve as a deep filter which extracts the pivotal information from the contaminated input spectrograms to counter the adversarial attacks.
% and protect anti-spoofing models in the black-box attack scenario.
%To the best of our knowledge, we are among the first ones to adopt the high-level representations extracted by the self-supervised model for the defense of anti-spoofing models in the black-box scenario and the experimental results show the effectiveness of our proposed method.
%We also propose the layerwise noise-to-signal ratio (LNSR), to quantize and measure the effect of deep models in countering adversarial noise.
%We find that the adversarial noise is attenuated layer by layer in the self-supervised learning model.

The paper is organized as follows. In Section 2, we firstly revisit the success of data augmentation method, and then introduce the background of adversarial attack and methods adopted in this paper, after that, we presents the proposed voting method. 
Section 4 reports the experimental setups, results, and analysis. Section 5 shows the conclusion.


